Are Neural Language Models Good Plagiarists? A Benchmark for Neural Paraphrase Detection

The rise of language models such as BERT allows for high-quality text paraphrasing. This is a problem to academic integrity, as it is difficult to differentiate between original and machine-generated content. We propose a benchmark consisting of paraphrased articles using recent language models relying on the Transformer architecture. Our contribution fosters future research of paraphrase detection systems as it offers a large collection of aligned original and paraphrased documents, a study regarding its structure, classification experiments with state-of-the-art systems, and we make our findings publicly available.

==> tables/full_dataset_stats_old.tex <==
\begin{table}[ht!]
\caption{Overview of the original paragraphs in our dataset.\label{tab:dataset-description}}
\resizebox{1\columnwidth}{!}{
\begin{threeparttable}
\centering
\begin{tabular}{clrrrr}
\toprule
                         &            & \textbf{arXiv}    & \textbf{Theses}   & \textbf{Wiki} & \textbf{Wiki-Train} \\ \midrule
\multirow{3}{*}{General} & Paragraphs & 20\,966    & 5\,226     & 39\,241     & 98\,282       \\
                         & \# Words   & 3\,194\,695  & 747\,545   & 5\;993\,461   & 17\,390\,048    \\
                         & Avg. Words & 152.38   & 143.04   & 152.73    & 176.94      \\ \midrule
\multirow{9}{*}{POS}     & NOUN       & 22.22\%  & 23.34\%  & 17.36\%   & 17.74\%     \\
                         & VERB       & 12.29\%  & 12.81\%  & 12.72\%   & 12.96\%     \\
                         & ADP        & 12.28\%  & 11.33\%  & 12.11\%   & 12.14\%     \\
                         & DET        & 12.03\%  & 10.14\%  & 10.08\%   & 10.13\%     \\
                         & PUNCT      & 11.58\%  & 11.80\%  & 13.61\%   & 13.31\%     \\
                         & ADJ        & 9.14\%   & 7.86\%   & 6.10\%    & 6.53\%      \\
                         & ADV        & 3.83\%   & 3.52\%   & 2.96\%    & 3.01\%      \\
                         & PROPN      & 3.74\%   & 4.88\%   & 12.35\%   & 11.43\%     \\
                         & OTHERS     & 12.90\%  & 14.32\%  & 12.71\%   & 12.76\%     \\ \cmidrule(lr){2-6}
                         & Total      & 100.00\% & 100.00\% & 100.00\%  & 100.00\%    \\ \midrule
\multirow{9}{*}{NER}     & CARDINAL   & 1.27\%   & 1.12\%   & 1.04\%    & 0.92\%      \\
                         & ORG        & 0.98\%   & 1.12\%   & 1.73\%    & 1.61\%      \\
                         & PERSON     & 0.48\%   & 0.42\%   & 2.13\%    & 2.03\%      \\
                         & DATE       & 0.26\%   & 1.00\%   & 1.56\%    & 1.51\%      \\
                         & GPE        & 0.22\%   & 0.67\%   & 1.17\%    & 1.16\%      \\
                         & ORDINAL    & 0.18\%   & 0.19\%   & 0.37\%    & 0.31\%      \\
                         & NORP       & 0.10\%   & 0.27\%   & 0.51\%    & 0.59\%      \\
                         & PERCENT    & 0.05\%   & 0.23\%   & 0.05\%    & 0.04\%      \\
                         & OTHERS     & 0.21\%   & 0.27\%   & 1.12\%    & 1.03\%      \\ \cmidrule(lr){2-6}
                         & Total      & 3.76\%   & 5.29\%   & 9.68\%    & 9.20\%  \\ \bottomrule   
\end{tabular}
\begin{tablenotes}
\item The table shows the NER and POS tags occurring most frequently in the original content from arXiv and theses (used to create the test sets) and Wikipedia (used to create the training and test sets). The values are ordered according to arXiv. OTHERS contains all tags not displayed. Please see our repository for a complete listing of all tags and their occurrence frequency in our dataset.
\end{tablenotes}
\end{threeparttable}
}
\end{table}

==> tables/named_entities.tex <==
\begin{table}[t!]
\caption{Overview of the average ignored tokens per paragraph.\label{tab:named-entities}}

\begin{threeparttable}
\centering
\begin{tabular}{lrrrr}
\toprule
\textbf{Named Entities} & \textbf{arXiv}    & \textbf{Theses}   & \textbf{Wiki} & \textbf{Wiki-Train} \\ \midrule
Cardinal   & 1.27\%   & 1.12\%   & 1.04\%    & 0.92\%      \\
Organization        & 0.98\%   & 1.12\%   & 1.73\%    & 1.61\%      \\
Person     & 0.48\%   & 0.42\%   & 2.13\%    & 2.03\%      \\
Date       & 0.26\%   & 1.00\%   & 1.56\%    & 1.51\%      \\
Geopolitical Entity         & 0.22\%   & 0.67\%   & 1.17\%    & 1.16\%      \\
Ordinal    & 0.18\%   & 0.19\%   & 0.37\%    & 0.31\%      \\
Nationalities/Political Groups       & 0.10\%   & 0.27\%   & 0.51\%    & 0.59\%      \\
Percent    & 0.05\%   & 0.23\%   & 0.05\%    & 0.04\%      \\
Others     & 0.21\%   & 0.27\%   & 1.12\%    & 1.03\%      \\ \cmidrule(lr){1-5}
Total      & 3.76\%   & 5.29\%   & 9.68\%    & 9.20\%  \\ \bottomrule   
\end{tabular}
\end{threeparttable}

\end{table}
